A hot mini-Neptune and a temperate, highly eccentric sub-Saturn around the bright K-dwarf TOI-2134

We present the characterisation of an inner mini-Neptune in a 9.2292005$\pm$0.0000063 day orbit and an outer mono-transiting sub-Saturn planet in a 95.50$^{+0.36}_{-0.25}$ day orbit around the moderately active, bright (mv=8.9 mag) K5V star TOI-2134. Based on our analysis of five sectors of TESS data, we determine the radii of TOI-2134b and c to be 2.69$\pm$0.16 R$_{e}$ for the inner planet and 7.27$\pm$0.42 R$_{e}$ for the outer one. We acquired 111 radial-velocity spectra with HARPS-N and 108 radial-velocity spectra with SOPHIE. After careful periodogram analysis, we derive masses for both planets via Gaussian Process regression: 9.13$^{+0.78}_{-0.76}$ M$_{e}$ for TOI-2134b and 41.86$^{+7.69}_{-7.83}$ M$_{e}$ for TOI-2134c. We analysed the photometric and radial-velocity data first separately, then jointly. The inner planet is a mini-Neptune with density consistent with either a water-world or a rocky core planet with a low-mass H/He envelope. The outer planet has a bulk density similar to Saturn's. The outer planet is derived to have a significant eccentricity of 0.67$^{+0.05}_{-0.06}$ from a combination of photometry and RVs. We compute the irradiation of TOI-2134c as 1.45$\pm$0.10 times the bolometric flux received by Earth, positioning it for part of its orbit in the habitable sone of its system. We recommend further RV observations to fully constrain the orbit of TOI-2134c. With an expected Rossiter-McLaughlin (RM) effect amplitude of 7.2$\pm$1.3 m/s, we recommend TOI-2134c for follow-up RM analysis to study the spin-orbit architecture of the system. We calculate the Transmission Spectroscopy Metric, and both planets are suitable for bright-mode NIRCam atmospheric characterisation.

==> Tables/table_HARPSN_data.tex <==
\begin{table*}

\caption{HARPS-N radial velocity and activity proxy data}
\label{tab:HN_data}
\begin{tabular}{llllllllllllllllll}
\hline
\hline
BJD - 2400000 & RV [m s$^{-1}$] & $\sigma_{\rm RV}$ [m s$^{-1}$] & FWHM [m s$^{-1}$] & $\sigma_{\rm FWHM}$ [m s$^{-1}$] & Contrast [\%]  & $\sigma_{\rm cont}$ [\%] & S-index & $\sigma_{\rm S-index}$\\
\hline
59416.60725662997  & -20611.611177 & 0.469509 & 5782.383494 & 0.939018  & 58.747433 & 0.009540      & 0.568103 & 0.000473 \\
59417.55154525023  & -20616.933652 & 0.574282 & 5784.631910 & 1.148563  & 58.756756 & 0.011666      & 0.563344 & 0.000661 \\
59418.571525949985 & -20621.390899 & 1.314713 & 5782.729884 & 2.629426  & 58.774429 & 0.026725      & 0.557175 & 0.002650 \\
59427.39696507016  & -20622.609950 & 0.651334 & 5786.836329 & 1.302668  & 58.729108 & 0.013220      & 0.592762 & 0.000813 \\
59428.6019380698   & -20620.606779 & 1.180816 & 5788.789450 & 2.361631  & 58.809633 & 0.023992      & 0.555585 & 0.002351 \\
59429.63629106991  & -20623.225562 & 0.850299 & 5790.512961 & 1.700597  & 58.762108 & 0.017258      & 0.579910 & 0.001374 \\
59430.565740869846 & -20622.131598 & 1.010224 & 5793.407987 & 2.020448  & 58.774393 & 0.020498      & 0.570431 & 0.001778 \\
59431.60472946009  & -20617.847534 & 0.840051 & 5792.981497 & 1.680101  & 58.737697 & 0.017035      & 0.599608 & 0.001348 \\
59443.52447101986  & -20632.464041 & 1.175767 & 5793.199755 & 2.351534  & 58.806771 & 0.023870      & 0.566712 & 0.002220 \\
59444.49848092999  & -20635.269577 & 0.908115 & 5785.739048 & 1.816229  & 58.790627 & 0.018455      & 0.585640 & 0.001443 \\
59445.54336798005  & -20637.634661 & 0.720225 & 5786.549441 & 1.440449  & 58.791224 & 0.014635      & 0.589600 & 0.000970 \\
59446.532862610184 & -20638.557726 & 0.536872 & 5779.897294 & 1.073745  & 58.790353 & 0.010922      & 0.585852 & 0.000592 \\
59447.550827569794 & -20636.523979 & 0.723476 & 5776.234892 & 1.446952  & 58.824233 & 0.014736      & 0.574713 & 0.001002 \\
59448.5388615001   & -20634.478526 & 0.601365 & 5770.719563 & 1.202729  & 58.852141 & 0.012266      & 0.565313 & 0.000727 \\
59449.5540507501   & -20631.946722 & 0.626438 & 5776.917752 & 1.252875  & 58.835000 & 0.012760      & 0.568733 & 0.000787 \\
59457.511907380074 & -20627.754594 & 0.595422 & 5767.489812 & 1.190844  & 58.887337 & 0.012159      & 0.555476 & 0.000706 \\
59458.50508393021  & -20628.217627 & 0.618309 & 5770.532974 & 1.236618  & 58.899031 & 0.012622      & 0.539781 & 0.000754 \\
59459.484949249774 & -20623.320754 & 0.749107 & 5768.276665 & 1.498213  & 58.923287 & 0.015304      & 0.532778 & 0.001050 \\
59461.49748940999  & -20623.083231 & 0.682538 & 5769.959341 & 1.365075  & 58.909818 & 0.013937      & 0.545323 & 0.000896 \\
59462.491892289836 & -20621.755087 & 0.577403 & 5770.450504 & 1.154805  & 58.872808 & 0.011782      & 0.557099 & 0.000669 \\
59464.492813929915 & -20626.240997 & 0.974741 & 5774.864122 & 1.949483  & 58.915060 & 0.019889      & 0.542209 & 0.001647 \\
59465.45167846978  & -20624.143710 & 0.643320 & 5777.111014 & 1.286640  & 58.838455 & 0.013104      & 0.554215 & 0.000789 \\
59472.47385834996  & -20611.885834 & 0.568317 & 5785.833212 & 1.136634  & 58.730955 & 0.011538      & 0.575649 & 0.000662 \\
59473.45919675985  & -20616.139827 & 1.209034 & 5787.770175 & 2.418069  & 58.836546 & 0.024581      & 0.556782 & 0.002355 \\
59475.46270379005  & -20616.083911 & 1.341184 & 5793.945516 & 2.682368  & 58.767772 & 0.027207      & 0.543373 & 0.002783 \\
59476.467913240194 & -20616.796905 & 0.891025 & 5785.980789 & 1.782050  & 58.759431 & 0.018098      & 0.558253 & 0.001477 \\
59477.44941222994  & -20612.133873 & 0.823639 & 5792.304963 & 1.647278  & 58.742204 & 0.016706      & 0.570220 & 0.001277 \\
59478.401417490095 & -20615.280319 & 0.791816 & 5789.232705 & 1.583632  & 58.739917 & 0.016068      & 0.554987 & 0.001142 \\
59479.4151798198   & -20616.253980 & 0.894083 & 5782.501817 & 1.788166  & 58.817868 & 0.018189      & 0.552986 & 0.001446 \\
59481.44507926982  & -20615.918136 & 0.933066 & 5780.449577 & 1.866132  & 58.857862 & 0.019001      & 0.557715 & 0.001553 \\
59513.328770080116 & -20611.664994 & 0.713992 & 5775.181762 & 1.427984  & 58.916978 & 0.014568      & 0.599082 & 0.001085 \\
59514.395987929776 & -20607.360769 & 0.615013 & 5780.850213 & 1.230025  & 58.864079 & 0.012525      & 0.606696 & 0.000883 \\
59515.32445032988  & -20606.725186 & 0.553245 & 5782.714142 & 1.106490  & 58.822188 & 0.011255      & 0.620149 & 0.000692 \\
59638.77612392977  & -20638.915373 & 0.989806 & 5753.404049 & 1.979612  & 59.116772 & 0.020341      & 0.534284 & 0.001840 \\
59642.77729215007  & -20635.000233 & 0.702654 & 5743.588209 & 1.405308  & 59.171449 & 0.014478      & 0.554961 & 0.001032 \\
59646.75007371977  & -20626.271999 & 0.602588 & 5756.198421 & 1.205176  & 59.078400 & 0.012369      & 0.585905 & 0.000800 \\
59647.7599757202   & -20627.602949 & 0.725069 & 5755.455617 & 1.450138  & 59.056380 & 0.014880      & 0.587636 & 0.001051 \\
59648.75532741984  & -20627.011824 & 0.621370 & 5759.687076 & 1.242739  & 58.984127 & 0.012727      & 0.582624 & 0.000821 \\
59649.753869649954 & -20625.407919 & 0.723276 & 5759.686546 & 1.446553  & 59.001970 & 0.014818      & 0.584261 & 0.001097 \\
59650.745116349775 & -20623.125169 & 0.511531 & 5765.271475 & 1.023063  & 58.903998 & 0.010453      & 0.584738 & 0.000592 \\
59651.7133117998   & -20621.916900 & 0.606053 & 5769.451652 & 1.212106  & 58.894268 & 0.012373      & 0.591673 & 0.000813 \\
59655.726336650085 & -20618.291484 & 0.893658 & 5777.780995 & 1.787316  & 58.870632 & 0.018211      & 0.596023 & 0.001542 \\
59656.760415070225 & -20620.202036 & 0.772589 & 5773.595380 & 1.545179  & 58.878812 & 0.015758      & 0.620998 & 0.001213 \\
59657.769726689905 & -20622.265292 & 0.896409 & 5771.831123 & 1.792818  & 58.829573 & 0.018273      & 0.610386 & 0.001524 \\
59658.739516729955 & -20622.450179 & 0.689101 & 5767.734331 & 1.378202  & 58.920426 & 0.014079      & 0.605825 & 0.001003 \\
59659.75800953992  & -20618.911301 & 0.634827 & 5762.537297 & 1.269653  & 58.937590 & 0.012986      & 0.598251 & 0.000868 \\
59660.74446539022  & -20618.082081 & 0.510132 & 5767.808129 & 1.020264  & 58.883294 & 0.010416      & 0.612355 & 0.000588 \\
59663.689832400065 & -20614.520190 & 0.573737 & 5768.076257 & 1.147473  & 58.933854 & 0.011724      & 0.602951 & 0.000737 \\
59682.75332385022  & -20613.907045 & 0.523633 & 5724.506616 & 1.047266  & 59.220122 & 0.010834      & 0.507489 & 0.000612 \\
59684.712612790056 & -20616.968946 & 0.827681 & 5726.210320 & 1.655362  & 59.302937 & 0.017144      & 0.487291 & 0.001377 \\
59685.71762247011  & -20620.118218 & 0.603735 & 5724.354724 & 1.207470  & 59.265793 & 0.012501      & 0.502977 & 0.000804 \\
59686.67411288014  & -20619.549105 & 1.388036 & 5725.519183 & 2.776071  & 59.174275 & 0.028691      & 0.476122 & 0.003212 \\
59704.73628506018  & -20618.703534 & 0.684879 & 5747.923901 & 1.369759  & 59.023128 & 0.014066      & 0.558752 & 0.000999 \\
59705.6778235198   & -20619.754614 & 0.972685 & 5754.710951 & 1.945371  & 59.126736 & 0.019988      & 0.558780 & 0.001728 \\
59706.69944042014  & -20617.978848 & 0.671338 & 5753.680490 & 1.342677  & 59.081028 & 0.013787      & 0.563133 & 0.000928 \\
59707.67638680013  & -20616.103253 & 0.906546 & 5751.478414 & 1.813091  & 59.130051 & 0.018640      & 0.566309 & 0.001632 \\
59708.67453762982  & -20615.727854 & 0.782089 & 5752.212813 & 1.564178  & 59.122683 & 0.016077      & 0.573023 & 0.001288 \\
59713.71820313996  & -20621.983030 & 0.789635 & 5752.083234 & 1.579271  & 59.111127 & 0.016229      & 0.552790 & 0.001257 \\
59714.69543228019  & -20622.725587 & 0.509178 & 5752.313542 & 1.018356  & 59.031165 & 0.010451      & 0.540256 & 0.000585 \\
59715.697339309845 & -20621.610778 & 0.521898 & 5753.605156 & 1.043796  & 59.043667 & 0.010711      & 0.523572 & 0.000611 \\
59716.67116793012  & -20622.031865 & 0.514032 & 5754.158828 & 1.028064  & 59.018704 & 0.010545      & 0.526647 & 0.000584 \\
59717.68496175017  & -20622.321355 & 0.428455 & 5749.943651 & 0.856910  & 59.046251 & 0.008800      & 0.526035 & 0.000433 \\
59718.62335636979  & -20623.640537 & 0.480521 & 5749.706122 & 0.961043  & 59.083422 & 0.009876      & 0.530079 & 0.000526 \\
\end{tabular}
\end{table*}
\newpage
\begin{table*}
\ContinuedFloat
\caption{HARPS-N radial velocity and activity proxy data (continued)}
\label{tab:HN_data2}
\begin{tabular}{llllllllllllllllll}
\hline
\hline
BJD - 2400000 & RV [m s$^{-1}$] & $\sigma_{\rm RV}$ [m s$^{-1}$] & FWHM [m s$^{-1}$] & $\sigma_{\rm FWHM}$ [m s$^{-1}$] & Contrast [\%]  & $\sigma_{\rm cont}$ [\%] & S-index & $\sigma_{\rm S-index}$\\
\hline
59719.71188513003  & -20625.678763 & 0.566118 & 5746.312053 & 1.132236  & 59.120286 & 0.011649      & 0.530654 & 0.000705 \\
59733.722817779984 & -20639.533275 & 0.516927 & 5726.708911 & 1.033854  & 59.238316 & 0.010694      & 0.476667 & 0.000612 \\
59737.63394954009  & -20635.025349 & 0.825963 & 5731.618635 & 1.651926  & 59.311420 & 0.017094      & 0.487193 & 0.001390 \\
59738.68015214987  & -20634.908266 & 1.104504 & 5728.694105 & 2.209007  & 59.413053 & 0.022910      & 0.450345 & 0.002218 \\
59739.663775700144 & -20634.859268 & 0.642563 & 5730.192403 & 1.285126  & 59.302250 & 0.013300      & 0.493849 & 0.000866 \\
59747.61815614998  & -20621.225054 & 1.001906 & 5748.551097 & 2.003812  & 59.179747 & 0.020629      & 0.511278 & 0.001863 \\
59748.66423752019  & -20622.729372 & 0.807197 & 5750.309060 & 1.614393  & 59.111935 & 0.016596      & 0.536285 & 0.001301 \\
59749.64699140983  & -20623.689462 & 0.822524 & 5750.141484 & 1.645047  & 59.108962 & 0.016910      & 0.548357 & 0.001336 \\
59750.62170770997  & -20626.476563 & 0.636422 & 5751.406447 & 1.272845  & 59.066946 & 0.013072      & 0.542814 & 0.000847 \\
59751.65170795005  & -20625.630448 & 0.498768 & 5749.383590 & 0.997535  & 59.030579 & 0.010242      & 0.537018 & 0.000563 \\
59752.62645826023  & -20624.044217 & 0.713225 & 5751.845981 & 1.426450  & 59.077616 & 0.014651      & 0.532089 & 0.001044 \\
59768.61528890021  & -20620.340975 & 0.739338 & 5742.087884 & 1.478675  & 59.171078 & 0.015237      & 0.511902 & 0.001129 \\
59769.597978719976 & -20621.235089 & 1.077096 & 5737.518939 & 2.154192  & 59.309646 & 0.022268      & 0.498464 & 0.002123 \\
59771.62816471979  & -20616.444301 & 0.711268 & 5732.807082 & 1.422535  & 59.228215 & 0.014697      & 0.510405 & 0.001119 \\
59772.629510459956 & -20616.339167 & 0.448861 & 5734.948967 & 0.897722  & 59.126671 & 0.009255      & 0.507424 & 0.000471 \\
59773.57368492009  & -20615.272526 & 0.461121 & 5733.211468 & 0.922242  & 59.142521 & 0.009514      & 0.502042 & 0.000482 \\
59774.56217591977  & -20615.261708 & 0.467405 & 5728.959983 & 0.934810  & 59.153431 & 0.009652      & 0.497366 & 0.000502 \\
59775.53706787992  & -20615.560839 & 0.719736 & 5733.432919 & 1.439471  & 59.199967 & 0.014863      & 0.483798 & 0.001067 \\
59788.51492572995  & -20623.914136 & 0.683509 & 5730.553167 & 1.367018  & 59.268780 & 0.014139      & 0.491076 & 0.000952 \\
59789.50055039022  & -20622.261331 & 0.740801 & 5729.351098 & 1.481603  & 59.304941 & 0.015336      & 0.497643 & 0.001124 \\
59801.48661554977  & -20615.268242 & 0.529333 & 5752.015203 & 1.058666  & 59.009471 & 0.010861      & 0.535654 & 0.000605 \\
59802.50195454992  & -20618.636971 & 0.503167 & 5752.174303 & 1.006334  & 59.032988 & 0.010328      & 0.531340 & 0.000556 \\
59803.510820759926 & -20621.208911 & 0.571101 & 5743.728352 & 1.142203  & 59.093858 & 0.011751      & 0.518980 & 0.000709 \\
59804.503320979886 & -20625.180449 & 0.561024 & 5739.392947 & 1.122047  & 59.137947 & 0.011561      & 0.523779 & 0.000691 \\
59805.478324079886 & -20627.260163 & 0.715086 & 5739.050215 & 1.430171  & 59.203448 & 0.014754      & 0.509572 & 0.001044 \\
59807.50367398979  & -20627.357661 & 0.642580 & 5731.814685 & 1.285159  & 59.244529 & 0.013284      & 0.497839 & 0.000878 \\
59808.529027369805 & -20625.709016 & 0.767696 & 5727.817850 & 1.535392  & 59.288035 & 0.015893      & 0.484566 & 0.001205 \\
59822.43823549012  & -20635.187440 & 0.785926 & 5730.393247 & 1.571852  & 59.267035 & 0.016257      & 0.476841 & 0.001240 \\
59828.42978822999  & -20632.374211 & 0.463050 & 5740.243361 & 0.926100  & 59.086576 & 0.009533      & 0.498037 & 0.000488 \\
59829.435602659825 & -20630.383876 & 0.570794 & 5740.759255 & 1.141589  & 59.114148 & 0.011755      & 0.505331 & 0.000708 \\
59830.44831448002  & -20630.743125 & 0.786416 & 5743.936727 & 1.572833  & 59.167109 & 0.016201      & 0.491324 & 0.001271 \\
59831.39873096999  & -20634.645979 & 0.601690 & 5743.078335 & 1.203379  & 59.115707 & 0.012387      & 0.512907 & 0.000776 \\
59832.43039386999  & -20635.151529 & 0.571127 & 5743.310220 & 1.142254  & 59.102662 & 0.011755      & 0.508248 & 0.000709 \\
59833.393588730134 & -20636.939191 & 0.600683 & 5743.733158 & 1.201366  & 59.082600 & 0.012358      & 0.513307 & 0.000773 \\
59834.397655739915 & -20639.084039 & 0.632077 & 5746.897682 & 1.264153  & 59.130137 & 0.013007      & 0.522131 & 0.000839 \\
59835.42387707019  & -20636.666663 & 0.605312 & 5746.975865 & 1.210623  & 59.116342 & 0.012453      & 0.523126 & 0.000779 \\
59836.41248239996  & -20632.252955 & 0.658880 & 5741.761633 & 1.317760  & 59.134198 & 0.013572      & 0.540536 & 0.000906 \\
59843.45019976003  & -20622.087429 & 0.762141 & 5746.639563 & 1.524282  & 59.073865 & 0.015669      & 0.552638 & 0.001201 \\
59844.41202594992  & -20622.314648 & 0.710251 & 5746.833366 & 1.420502  & 59.053145 & 0.014597      & 0.532303 & 0.001044 \\
59845.41189453984  & -20621.941218 & 0.708613 & 5746.281563 & 1.417226  & 59.048920 & 0.014563      & 0.527358 & 0.001044 \\
59858.35123518016  & -20618.879264 & 0.921107 & 5723.763488 & 1.842215  & 59.317613 & 0.019092      & 0.487907 & 0.001495 \\
59859.37847934989  & -20620.251551 & 0.615232 & 5727.862262 & 1.230465  & 59.236443 & 0.012725      & 0.481582 & 0.000809 \\
59860.35796819022  & -20621.461814 & 0.921100 & 5729.844188 & 1.842199  & 59.266199 & 0.019055      & 0.466630 & 0.001626 \\
59861.35995269008  & -20621.442640 & 0.662220 & 5730.313691 & 1.324440  & 59.188671 & 0.013680      & 0.479048 & 0.000917 \\
59865.35989473993  & -20614.634687 & 1.384556 & 5738.503426 & 2.769112  & 59.270610 & 0.028601      & 0.514982 & 0.003253 \\
59869.380423599854 & -20622.262238 & 0.889023 & 5730.999430 & 1.778045  & 59.271531 & 0.018389      & 0.475346 & 0.001565 \\
59871.35436584009  & -20622.399823 & 0.729163 & 5728.194772 & 1.458326  & 59.288424 & 0.015094      & 0.486457 & 0.001088 \\
59872.32706419006  & -20619.733613 & 0.738026 & 5727.640099 & 1.476053  & 59.288416 & 0.015279      & 0.492316 & 0.001069 \\
59890.32938627992  & -20618.962886 & 0.581073 & 5727.937335 & 1.162147  & 59.174230 & 0.012006      & 0.496025 & 0.000738 \\
59892.3217106699   & -20616.622849 & 0.557809 & 5724.807364 & 1.115619  & 59.187096 & 0.011534      & 0.492493 & 0.000661
\end{tabular}
\end{table*}

==> Tables/table_SOPHIE_act.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}
\caption{SOPHIE RV activity proxy data \label{tab:SP_act}}
\begin{tabular}{llll}
\hline
\hline
BJD - 2400000         & FWHM [km s$^{-1}$] & Contrast [\%] & BISS [km s$^{-1}$]) \\
\hline
59082.35826 & 7.11       & 42.59    & 0.004      \\
59085.39497 & 7.11       & 42.48    & 0.023      \\
59108.31091 & 7.11       & 42.24    & 0.002      \\
59110.35828 & 7.10       & 42.39    & 0.018      \\
59111.31119 & 7.09       & 42.13    & 0.002      \\
59113.39451 & 7.08       & 42.44    & 0.010      \\
59114.38395 & 7.11       & 42.37    & 0.016      \\
59116.31690 & 7.08       & 42.64    & 0.015      \\
59118.33599 & 7.07       & 42.25    & 0.005      \\
59128.34014 & 7.12       & 42.33    & 0.009      \\
59131.25440 & 7.08       & 42.82    & 0.024      \\
59132.25712 & 7.10       & 42.68    & 0.021      \\
59133.30482 & 7.11       & 42.41    & 0.017      \\
59134.33841 & 7.13       & 41.86    & 0.015      \\
59139.27625 & 7.05       & 42.90    & 0.028      \\
59140.37037 & 7.21       & 41.96    & 0.027      \\
59141.30968 & 7.09       & 42.54    & 0.019      \\
59147.32339 & 7.18       & 41.42    & 0.031      \\
59150.33084 & 7.21       & 42.11    & 0.009      \\
59166.28753 & 7.19       & 42.36    & 0.003      \\
59171.25381 & 7.19       & 42.12    & 0.019      \\
59172.22943 & 7.12       & 42.61    & 0.011      \\
59174.26200 & 7.16       & 42.30    & 0.004      \\
59176.22502 & 7.14       & 42.58    & 0.012      \\
59183.21627 & 7.21       & 42.25    & 0.025      \\
59303.64096 & 7.10       & 42.64    & 0.018      \\
59327.63050 & 7.11       & 42.99    & 0.014      \\
59329.57494 & 7.10       & 42.49    & 0.026      \\
59336.55162 & 7.12       & 42.44    & 0.022      \\
59337.54996 & 7.12       & 42.68    & 0.013      \\
59340.59837 & 7.12       & 42.64    & 0.019      \\
59343.60871 & 7.12       & 42.19    & 0.024      \\
59362.51191 & 7.09       & 42.88    & 0.024      \\
59394.59832 & 7.13       & 42.69    & 0.012      \\
59404.52885 & 7.09       & 42.41    & 0.007      \\
59405.53347 & 7.10       & 42.71    & 0.021      \\
59406.55399 & 7.11       & 42.29    & 0.018      \\
59418.36707 & 7.13       & 42.14    & 0.019      \\
59421.40970 & 7.12       & 42.39    & 0.017      \\
59422.51828 & 7.15       & 42.02    & 0.009      \\
59440.43363 & 7.12       & 42.31    & 0.013      \\
59445.44429 & 7.12       & 42.55    & 0.020      \\
59452.41120 & 7.11       & 42.29    & 0.034      \\
59455.44905 & 7.11       & 42.10    & 0.017      \\
59456.34748 & 7.09       & 43.08    & 0.010      \\
59457.45992 & 7.13       & 42.30    & 0.026      \\
59468.42133 & 7.11       & 42.14    & 0.015      \\
59469.43457 & 7.14       & 42.06    & 0.025      \\
59475.30015 & 7.11       & 42.27    & 0.005      \\
59485.28794 & 7.07       & 42.60    & 0.027      \\
59500.31460 & 7.12       & 42.46    & 0.001      \\
59502.27127 & 7.09       & 42.53    & 0.011      \\
59503.31929 & 7.09       & 42.37    & 0.017      \\
59505.26740 & 7.09       & 42.49    & 0.016      \\
59506.28444 & 7.10       & 42.48    & 0.023      \\
59511.28603 & 7.13       & 42.43    & 0.009      \\
59523.25390 & 7.14       & 42.09    & 0.014      \\
59525.23651 & 7.15       & 42.46    & 0.016      \\
59623.71838 & 7.13       & 42.65    & 0.021      \\
59629.68179 & 7.10       & 41.65    & 0.014      \\
59646.69203 & 7.12       & 42.30    & 0.002      \\
59660.61030 & 7.14       & 42.15    & 0.022      \\
59662.60824 & 7.12       & 42.21    & 0.010      \\
59663.58011 & 7.15       & 42.09    & 0.017      \\
\end{tabular}
\end{table}

\begin{table}
\ContinuedFloat
\caption{SOPHIE RV activity proxy data (continued) \label{tab:SP_act2}}
\begin{tabular}{llll}
\hline
\hline
BJD-2400000         & FWHM [km s$^{-1}$] & Contrast [\%] & BISS [km s$^{-1}$] \\
\hline
59683.59294 & 7.08       & 42.74    & 0.011      \\
59685.58630 & 7.09       & 42.62    & 0.016      \\
59687.65374 & 7.11       & 42.27    & -0.003     \\
59712.49299 & 7.10       & 42.58    & 0.013      \\
59717.50957 & 7.12       & 42.39    & 0.020      \\
59728.54292 & 7.09       & 42.39    & 0.013      \\
59729.48571 & 7.07       & 42.78    & 0.031      \\
59751.58025 & 7.10       & 42.56    & 0.008      \\
59753.58004 & 7.11       & 42.61    & 0.032      \\
59773.51577 & 7.08       & 42.02    & -0.001     \\
59782.35626 & 7.09       & 42.80    & 0.003      \\
59782.51887 & 7.09       & 42.68    & 0.011      \\
59783.39302 & 7.11       & 42.63    & 0.024      \\
59783.55408 & 7.13       & 42.54    & 0.017      \\
59784.42100 & 7.08       & 42.69    & 0.014      \\
59784.50001 & 7.10       & 42.72    & 0.017      \\
59785.40799 & 7.08       & 42.92    & 0.005      \\
59785.55282 & 7.11       & 42.80    & 0.018      \\
59786.55851 & 7.12       & 42.30    & 0.025      \\
59787.36459 & 7.07       & 42.65    & 0.014      \\
59787.50217 & 7.09       & 42.71    & 0.034      \\
59806.39184 & 7.10       & 42.37    & 0.023      \\
59806.49052 & 7.13       & 42.10    & 0.013      \\
59808.32652 & 7.08       & 42.47    & 0.003      \\
59813.41619 & 7.08       & 42.54    & 0.003      \\
59814.43468 & 7.06       & 41.59    & 0.010      \\
59824.36774 & 7.08       & 42.81    & 0.020      \\
59882.24495 & 7.07       & 41.96    & -0.013     \\
59889.24966 & 7.10       & 42.13    & 0.019      \\
59894.23454 & 7.11       & 42.41    & 0.001     
\end{tabular}
\end{table}

==> Tables/table_SOPHIE_data.tex <==
% Please add the following required packages to your document preamble:
%\usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}
\caption{SOPHIE radial velocity data \label{tab:SP_data}}
\begin{tabular}{lll}
\hline
\hline
BJD - 2400000 & RV [km s$^{-1}$]    & $\sigma_{RV}$ [km s$^{-1}$]\\
\hline
59082.35826 & -20.6245 & 0.0021 \\
59085.39497 & -20.6313 & 0.0021 \\
59108.31091 & -20.6237 & 0.0021 \\
59110.35828 & -20.6234 & 0.0021 \\
59111.31119 & -20.6300 & 0.0022 \\
59113.39451 & -20.6355 & 0.0021 \\
59114.38395 & -20.6390 & 0.0021 \\
59116.31690 & -20.6353 & 0.0021 \\
59118.33599 & -20.6222 & 0.0024 \\
59119.36516 & -20.6296 & 0.0030 \\
59128.34014 & -20.6209 & 0.0021 \\
59131.25440 & -20.6256 & 0.0021 \\
59132.25712 & -20.6325 & 0.0021 \\
59133.30482 & -20.6266 & 0.0021 \\
59139.27625 & -20.6383 & 0.0021 \\
59140.37037 & -20.6495 & 0.0020 \\
59141.30968 & -20.6427 & 0.0021 \\
59147.32339 & -20.6387 & 0.0025 \\
59150.33084 & -20.6534 & 0.0021 \\
59152.26399 & -20.6287 & 0.0040 \\
59166.28753 & -20.6476 & 0.0020 \\
59171.25381 & -20.6515 & 0.0021 \\
59172.22943 & -20.6407 & 0.0021 \\
59174.26200 & -20.6354 & 0.0021 \\
59176.22502 & -20.6262 & 0.0021 \\
59180.21274 & -20.6351 & 0.0030 \\
59183.21627 & -20.6318 & 0.0021 \\
59303.64096 & -20.6248 & 0.0021 \\
59327.63050 & -20.6369 & 0.0021 \\
59329.57494 & -20.6242 & 0.0022 \\
59336.55162 & -20.6330 & 0.0022 \\
59337.54996 & -20.6405 & 0.0022 \\
59340.59837 & -20.6409 & 0.0022 \\
59343.60871 & -20.6424 & 0.0027 \\
59362.51191 & -20.6485 & 0.0020 \\
59392.52729 & -20.6294 & 0.0030 \\
59394.59832 & -20.6261 & 0.0021 \\
59404.52885 & -20.6315 & 0.0022 \\
59405.53347 & -20.6195 & 0.0021 \\
59406.55399 & -20.6211 & 0.0021 \\
59418.36707 & -20.6357 & 0.0022 \\
59419.45549 & -20.6288 & 0.0040 \\
59421.40970 & -20.6277 & 0.0021 \\
59422.51828 & -20.6296 & 0.0022 \\
59439.47283 & -20.6468 & 0.0030 \\
59440.43363 & -20.6419 & 0.0021 \\
59445.44429 & -20.6490 & 0.0021 \\
59452.41120 & -20.6434 & 0.0021 \\
59455.44905 & -20.6398 & 0.0021 \\
59456.34748 & -20.6491 & 0.0016 \\
59457.45992 & -20.6433 & 0.0021 \\
59468.42133 & -20.6311 & 0.0021 \\
59469.43457 & -20.6293 & 0.0021 \\
59475.30015 & -20.6312 & 0.0021 \\
59477.41895 & -20.6261 & 0.0030 \\
59485.28794 & -20.6353 & 0.0021 \\
59500.31460 & -20.6336 & 0.0021 \\
59502.27127 & -20.6338 & 0.0021 \\
\end{tabular}
\end{table}

\begin{table}
\ContinuedFloat
\caption{SOPHIE radial velocity data (continued) \label{tab:SP_data2}}
\begin{tabular}{lll}
\hline
\hline
BJD - 2400000 & RV [km s$^{-1}$]    & $\sigma_{RV}$ [km s$^{-1}$]\\
\hline
59503.31929 & -20.6307 & 0.0021 \\
59505.26740 & -20.6263 & 0.0021 \\
59506.28444 & -20.6202 & 0.0021 \\
59511.28603 & -20.6297 & 0.0021 \\
59523.25390 & -20.6245 & 0.0022 \\
59525.23651 & -20.6326 & 0.0017 \\
59623.71838 & -20.6433 & 0.0016 \\
59627.66855 & -20.6450 & 0.0030 \\
59629.68179 & -20.6442 & 0.0027 \\
59631.63954 & -20.6425 & 0.0030 \\
59646.69203 & -20.6387 & 0.0021 \\
59660.61030 & -20.6295 & 0.0019 \\
59662.60824 & -20.6274 & 0.0021 \\
59663.58011 & -20.6238 & 0.0021 \\
59683.59294 & -20.6265 & 0.0021 \\
59685.58630 & -20.6288 & 0.0021 \\
59686.61945 & -20.6293 & 0.0040 \\
59687.65374 & -20.6358 & 0.0020 \\
59712.49299 & -20.6265 & 0.0021 \\
59714.51657 & -20.6296 & 0.0030 \\
59715.52315 & -20.6333 & 0.0030 \\
59717.50957 & -20.6304 & 0.0021 \\
59728.54292 & -20.6385 & 0.0023 \\
59729.48571 & -20.6474 & 0.0021 \\
59751.58025 & -20.6372 & 0.0021 \\
59753.58004 & -20.6339 & 0.0021 \\
59770.52988 & -20.6361 & 0.0040 \\
59773.51577 & -20.6305 & 0.0022 \\
59782.35626 & -20.6262 & 0.0021 \\
59782.51887 & -20.6277 & 0.0021 \\
59783.39302 & -20.6266 & 0.0022 \\
59783.55408 & -20.6272 & 0.0021 \\
59784.42100 & -20.6272 & 0.0021 \\
59784.50001 & -20.6252 & 0.0021 \\
59785.40799 & -20.6275 & 0.0021 \\
59785.55282 & -20.6308 & 0.0021 \\
59786.55851 & -20.6330 & 0.0022 \\
59787.36459 & -20.6406 & 0.0023 \\
59787.50217 & -20.6359 & 0.0022 \\
59804.52010 & -20.6306 & 0.0040 \\
59806.39184 & -20.6434 & 0.0022 \\
59806.49052 & -20.6425 & 0.0022 \\
59808.32652 & -20.6461 & 0.0021 \\
59813.41619 & -20.6343 & 0.0021 \\
59814.43468 & -20.6409 & 0.0022 \\
59824.36774 & -20.6536 & 0.0021 \\
59881.25183 & -20.6280 & 0.0030 \\
59882.24495 & -20.6188 & 0.0027 \\
59889.24966 & -20.6379 & 0.0022 \\
59894.23454 & -20.6352 & 0.0021
\end{tabular}
\end{table}


==> Tables/table_act_gp.tex <==
\begin{table}
\centering
% \scriptsize
% \tablewidth{5pt}

\caption{Results of the staller activity proxies GP regression analysis. \label{bigtable}\label{tab:actgp}}

\begin{tabular}{cccc}

% Parameter & Notation & Prior\\
\rule{0pt}{0ex} \\
\hline
\hline
\rule{0pt}{0ex} \\

Parameter & HARPS-N S-index & SOPHIE bisector & Prior \\
\rule{0pt}{0ex} \\
\hline
\rule{0pt}{0ex}

$\theta_1$&value&value& $\mathcal{U}$(0,1) \\
$\theta_2$&value&value& $\mathcal{J}$(0,100)\\
$\theta_3$&value&value& $\mathcal{J}$(0,100) \\
$\theta_4$&value&value& $\mathcal{G}$(0.5,0.05)\\
Jitter & value&value & $\mathcal{U}$(0,1)\\


\rule{0pt}{0ex} \\
\hline
\rule{0pt}{0ex} \\


\end{tabular}
\end{table}

==> Tables/table_separategp.tex <==
\begin{table*}
\centering
% \scriptsize
\caption{Results from the three Gaussian Process regression analysis. In order the combined HARPS-N and SOPHIE data (used for all further analysis), the HARPS-N only, and the SOPHIE only results. We abbreviated uniform priors as $\mathcal{U}$, Gaussian priors as $\mathcal{G}$ and Jeffreys' priors as $\mathcal{J}$. \label{tab:separategp}}
% \tablewidth{5pt}

\begin{tabular}{ccc}

\hline
\hline\\[-5pt]

Parameter & Value & Prior \\ [4pt]

\hline\\[-5pt]


\multicolumn{3}{c}{\textbf{HARPS-N and SOPHIE combined analysis}}\\ [4pt]

    GP Amplitude $\theta_1$ [\ms] & \Kk$_{\Kkd}^{\Kku}$  & $\mathcal{U}[0,20]$\\ [2pt]
    GP Timescale $\theta_2$ [days] & \Evok$_{\Evokd}^{\Evoku}$ & $\mathcal{J}[0,100]$\\ [2pt]
    GP Period $\theta_3$ [days] & \Pk$_{\Pkd}^{\Pku}$ & $\mathcal{G}[48,10$]\\ [2pt]
    GP Smoothness $\theta_4$ & \Harmk$_{\Harmkd}^{\Harmku}$ & $\mathcal{G}[0.5,0.05]$\\ [2pt]
    Jitter [\ms] & \jit$_{\jitd}^{\jitu}$ & $\mathcal{U}[0,2]$\\ [2pt]
    SOPHIE - HARPS-N Offset [\ms] & \offset$_{\offsetd}^{\offsetu}$ & $\mathcal{U}[-5,5]$\\ [2pt]
    Orbital period $P_b$~[days] & 9.2292002$_{-0.0000041}^{+0.0000047}$ & $\mathcal{G}[9.2292309,0.0000371]$\\ [2pt]
    RV Amplitude $K_b$ [\ms] & \Kb$_{\Kbd}^{\Kbu}$ & $\mathcal{U}[0,20]$\\ [2pt]
    $S_{\rm k,b}$ & \Skb$_{\Skbd}^{\Skbu}$ & $\mathcal{U}[-1,1]$\\ [2pt]
    $C_{\rm k,b}$ & \Ckb$_{\Ckbd}^{\Ckbu}$ & $\mathcal{U}[-1,1]$\\ [2pt]
    Time of periastron $t_{\rm peri,b}$ [BJD] & 2459407.544935071$_{-0.000010}^{+0.000013}$ & $\mathcal{G}[2459408.227369, 0.000228]$\\ [2pt]
    Orbital period $P_c$~[days] & \Pc$_{\Pcd}^{\Pcu}$ & $\mathcal{G}[95,10]$\\ [2pt]
    RV Amplitude $K_c$ [\ms] & \Kc$_{\Kcd}^{\Kcu}$ & $\mathcal{U}[0,20]$\\ [2pt]
    $S_{\rm k,c}$ & \Skc$_{\Skcd}^{\Skcu}$ & $\mathcal{U}[-1,1]$\\[2pt]
    $C_{\rm k,c}$ &\Ckc$_{\Ckcd}^{\Ckcu}$ & $\mathcal{U}[-1,1]$\\ [2pt]
    Time of periastron $t_{\rm peri,c}$ [BJD] & \tperic$_{\tpericd}^{\tpericu}$ & $\mathcal{U}[2459678.5,2459773.5]$\\[4pt]

\hline\\[-5pt]

\multicolumn{3}{c}{\textbf{HARPS-N analysis}}\\[4pt]

    GP Amplitude $\theta_1$ [\ms] & 5.79$_{-1.10}^{+1.60}$  & $\mathcal{U}[0,20]$\\ [2pt]
    GP Timescale $\theta_2$ [days] & 35.75$_{-17.52}^{+11.55}$ & $\mathcal{J}[0,100]$\\ [2pt]
    GP Period $\theta_3$ [days] & 51$_{-6.72}^{+10.61}$ & $\mathcal{G}[48,10$]\\ [2pt]
    GP Smoothness $\theta_4$ & 0.50$_{-0.04}^{+0.03}$ & $\mathcal{G}[0.5,0.05]$\\ [2pt]
    Jitter [\ms] & 0.72$_{-0.16}^{+0.16}$ & $\mathcal{U}[0,2]$\\ [2pt]
    Orbital period $P_b$~[days] & 9.2292086$_{-0.000100}^{+0.000098}$ & $\mathcal{G}[9.2292309,0.0000371]$\\ [2pt]
    RV Amplitude $K_b$ [\ms] & 3.00$_{-0.46}^{+0.44}$ & $\mathcal{U}[0,20]$\\ [2pt]
    $S_{\rm k,b}$ & 0.00$_{-0.01}^{+0.01}$ & $\mathcal{U}[-1,1]$\\ [2pt]
    $C_{\rm k,b}$ & 0.01$_{-0.02}^{+0.06}$ & $\mathcal{U}[-1,1]$\\ [2pt]
    Time of periastron $t_{\rm peri,b}$ [BJD] & 2459407.54489$_{-0.0023}^{+0.0031}$ & $\mathcal{G}[2459408.227369, 0.000228]$\\ [2pt]
    Orbital period $P_c$~[days] & 96.08$_{-4.41}^{+4.25}$ & $\mathcal{G}[95,10]$\\ [2pt]
    RV Amplitude $K_c$ [\ms] & 6.57$_{-3.49}^{+2.83}$ & $\mathcal{U}[0,20]$\\ [2pt]
    $S_{\rm k,c}$ & 0.00$_{-0.01}^{+0.02}$ & $\mathcal{U}[-1,1]$\\[2pt]
    $C_{\rm k,c}$ & 0.01$_{-0.02}^{+0.08}$ & $\mathcal{U}[-1,1]$\\ [2pt]
    Time of periastron $t_{\rm peri,c}$ [BJD] & 2459718.6$_{-2.5}^{+3.2}$ & $\mathcal{U}[2459678.5,2459773.5]$\\[4pt]

\hline\\[-5pt]

\multicolumn{3}{c}{\textbf{SOPHIE analysis}}\\ [4pt]


    GP Amplitude $\theta_1$ [\ms] & 6.94$_{-1.18}^{+1.50}$  & $\mathcal{U}[0,20]$\\ [2pt]
    GP Timescale $\theta_2$ [days] & 10.15$_{-7.99}^{+22.51}$ & $\mathcal{J}[0,100]$\\ [2pt]
    GP Period $\theta_3$ [days] & 40.88$_{-22.50}^{+22.53}$ & $\mathcal{G}[48,10$]\\ [2pt]
    GP Smoothness $\theta_4$ & 0.49$_{-0.07}^{+0.06}$ & $\mathcal{G}[0.5,0.05]$\\ [2pt]
    Jitter [\ms] & 0.77$_{-0.24}^{+0.27}$ & $\mathcal{U}[0,2]$\\ [2pt]
    Orbital period $P_b$~[days] & 9.229206$_{-0.000067}^{+0.000083}$ & $\mathcal{G}[9.2292309,0.0000371]$\\ [2pt]
    RV Amplitude $K_b$ [\ms] & 3.43$_{-1.13}^{+1.19}$ & $\mathcal{U}[0,20]$\\ [2pt]
    $S_{\rm k,b}$ & 0.00$_{-0.01}^{+0.02}$ & $\mathcal{U}[-1,1]$\\ [2pt]
    $C_{\rm k,b}$ & 0.01$_{-0.03}^{+0.06}$ & $\mathcal{U}[-1,1]$\\ [2pt]
    Time of periastron $t_{\rm peri,b}$ [BJD] & 2459407.54486$_{-0.00015}^{+0.00031}$ & $\mathcal{G}[2459408.227369, 0.000228]$\\ [2pt]
    Orbital period $P_c$~[days] & 96.98$_{-1.65}^{+1.46}$ & $\mathcal{G}[95,10]$\\ [2pt]
    RV Amplitude $K_c$ [\ms] & 6.74$_{-2.81}^{+2.20}$ & $\mathcal{U}[0,20]$\\ [2pt]
    $S_{\rm k,c}$ & 0.02$_{-0.02}^{+0.04}$ & $\mathcal{U}[-1,1]$\\[2pt]
    $C_{\rm k,c}$ & 0.33$_{-0.06}^{+0.12}$ & $\mathcal{U}[-1,1]$\\ [2pt]
    Time of periastron $t_{\rm peri,c}$ [BJD] & 2459718.990893157$_{-0.86}^{+0.070}$ & $\mathcal{U}[2459678.5,2459773.5]$\\[4pt]
    
\hline


\end{tabular}	
\end{table*}

==> Tables/table_template.tex <==
\begin{table*}[]
\centering
% \scriptsize
\caption{System Parameters for the \thisstar\ system. \label{bigtable}\label{tab:star}}
% \tablewidth{5pt}

\begin{tabular}{ccc}
% Parameter & Notation & Prior\\
\rule{0pt}{0ex} \\
\hline
\hline
\rule{0pt}{0ex} \\


Parameter & Value & Source \\
\rule{0pt}{0ex} \\
\hline



	RA [h m s]      & 19 06 45.44 &  a \\
	DEC [d m s]     & +39 12 42.63 & a \\
	Spectral type   & G0V  \\
	$m_V$   & 11.05$\pm$0.08 &a \\
	$B-V$   & 0.57 & a\\
	Parallax [mas]  & 4.34$\pm$  0.53 & b \\
	Distance [pc]   & 230.41$\pm$ 28.14 & \\
	$T_{\rm eff}$ [K]  & 6148$\pm$ 71 & c \\
	$\log{g}$       & 4.36$\pm$ 0.10 & c \\
	${\rm [Fe/H]}$  &$-$0.24$\pm$ 0.05 & c \\
	$\Delta\nu$ [$\mu$Hz] & 128.8$\pm$ 1.3 & d \\
	$\nu_{max}$ [$\mu$Hz] & 2928.0$\pm$ 97.0 & d \\
	Mass $[M_{\odot}]$ & 1.03$\pm$ 0.04 & e \\
	Radius $[R_{\odot}]$ & 1.03$\pm$ 0.02 & e \\
	$\rho_{\ast}$ [$\rho_{\odot}$] & 0.94$\pm$ 0.04 & \\
    Age [Gyr] & 2.56$\pm$1.06 & e \\
	$v\,\sin{i}$ [km~s$^{-1}$]      & 3.5$\pm$ 0.5 & d \\

    Limb darkening $q_1$~ & $\ldone$ $\pm$ $ \uldone$ & f \\
    Limb darkening $q_2$~ & $\ldtwo$ $\pm$ $ \uldtwo$ & f \\	

	$<\log{R'_{\rm HK}}>$ & $-$4.97 & g \\
% 	P$_{\rm rot}$ [days] & $\prot$  $\pm$  $\prote$ & Huber 2013 \\

	P$_{\rm rot}$ [days] & $\prot$  $\pm$  $\prote$ & f \\
	$\tau_{\rm ev}$ [days] & $\tev$ $\pm$  $\teve$ & f \\
%	Systemic velocity $\gamma~(\ms)$ & $-20926.9^{+0.54}_{-0.64}$ & d \\



\hline

\emph{Transit and radial-velocity parameters} & & \\
    Orbital period $P$~[days] & $\perplb$  $\pm$ $ \uperplb $ & f \\
    Time of mid-transit $t_{0}$~[BJD] & $\ttransitb$  $\pm$ \uttransitb & f\\ 
    Radius ratio $(R_b/R_\star)$ & $\rprstb$   $\pm$ $ \urprstb$ & f \\
    Orbital inclination $i$~[deg] & $\inclb$   $\pm$ $ \uinclb$ & f \\ 
    Transit impact parameter $b$ & $\impb$   $\pm$ $ \uimpb$ & f \\
    RV semi-amplitude $K$ [m.s$^{-1}$] & $\kamp$   $\pm$ $ ^{\kampeu} _{-\kampel}$ & g \\
    RV semi-amplitude 68\% (95\%) upper limit [m.s$^{-1}$] & $<1.8$ ($<2.8$) & g \\
    % RV semi-amplitude 95\% upper limit [m.s$^{-1}$] & $<2.8$ & 8 \\
    % Eccentricity 68\% upper limit (from transit fit) &$<0.31$ & f \\
    Eccentricity 68\% (95\%) upper limit &$<0.36$ ($<0.79$)& g \\  
    Argument of periastron $\omega_p$ [deg] & -71 $\pm$ 92 & g \\
    RV offset RV$_0$ [km.s$^{-1}$]   & -40.6386 $\pm$ 0.000006 & g \\
    
    % $e_{68\%}<0.31$ and $e_{95\%}<0.71$
                              
\hline

\emph{Derived parameters for \thisplanet} & & \\
    Radius $R_b$~[\rearth] & $\rplb$     $\pm$ $ \urplb$  & e,f \\
    Mass $M_b$~[\mearth] & $\mass$     $\pm$ $ ^{\masseu} _{-\massel}$  & e,f,g \\
    Mass 68\% (95\%) upper limit [\mearth] & $< 6.2$ ($< \mupp$) &        e,f,g \\
    % Mass 95\% upper limit [\mearth] & $< \mupp$ &        6,f,8 \\
    Density $\rho_b$~[g.cm$^{-1}$] & $\rhopl$    $\pm$  $^{\rhopleu} _{-\rhoplel}$  & e,f,g \\
    Density 68\% (95\%) upper limit [g.cm$^{-1}$] & $< 3.2$  ($< 5.1$)  & e,f,g \\
    Scaled semi-major axis $a/R_\star$  & $\arstb$   $\pm$ $\uarstb$ & f \\
    Semi-major axis $a_b$ [AU] & 0.103 $\pm$ 0.001 & f, g \\
    Incident flux $F$~[\fearth] & $\flux$   $\pm$  $\fluxe$  & e,f \\
    



\rule{0pt}{0ex} \\
\hline
\rule{0pt}{0ex} \\

\end{tabular}

 
	\tablenotetext{1}{\cite{Hog2000}}
	\tablenotetext{2}{\cite{Gaia2016}}
	\tablenotetext{3}{from ARES+MOOG analysis, with the surface gravity corrected following \cite{Mortier2014}}
	\tablenotetext{4}{\cite{Huber2013}}
	\tablenotetext{5}{Bayesian estimation using the PARSEC isochrones and asteroseismology}
	\tablenotetext{6}{Analysis of the $Kepler$ lightcurve}
	\tablenotetext{7}{Analysis of the HARPS-N spectra/RVs}

\end{table*}







% \begin{deluxetable*}{lllll}
% \tablecaption{System Parameters for \thisstar \label{bigtable}\label{tab:star}}
% \tablewidth{0pt}
% \tablehead{
%   \colhead{Parameter} & 
%   \colhead{Value}     &
%   \colhead{} &
%   \colhead{Source}   \\
%   \colhead{} & 
%   \colhead{}     &
%   \colhead{} &
%   \colhead{}  
% }
% \startdata
% \emph{Parameters of the host star} & & \\




% 	RA [h m s]      & 19 06 45.44 &  1 \\
% 	DEC [d m s]     & +39 12 42.63 & 1 \\
% 	Spectral type   & G0V  \\
% 	$m_V$   & 11.05$\pm$0.08 &1 \\
% 	$B-V$   & 0.57 & 1\\
% 	Parallax [mas]  & 4.34$\pm$  0.53 & 2 \\
% 	Distance [pc]   & 230.41$\pm$ 28.14 & \\
% 	$T_{\rm eff}$ [K]  & 6148$\pm$ 71 & 3 \\
% 	$\log{g}$       & 4.36$\pm$ 0.10 & 3 \\
% 	${\rm [Fe/H]}$  &$-$0.24$\pm$ 0.05 & 3 \\
% 	$\Delta\nu$ [$\mu$Hz] & 128.8$\pm$ 1.3 & 5 \\
% 	$\nu_{max}$ [$\mu$Hz] & 2928.0$\pm$ 97.0 & 5 \\
% 	Mass $[M_{\odot}]$ & 1.03$\pm$ 0.04 & 6 \\
% 	Radius $[R_{\odot}]$ & 1.03$\pm$ 0.02 & 6 \\
% 	$\rho_{\ast}$ [$\rho_{\odot}$] & 0.94$\pm$ 0.04 & \\
%     Age [Gyr] & 2.56$\pm$1.06 & 6 \\
% 	$v\,\sin{i}$ [km~s$^{-1}$]      & 3.5$\pm$ 0.5 & 5 \\

%     Limb darkening $q_1$~ & $\ldone$ $\pm$ $ \uldone$ & 7 \\
%     Limb darkening $q_2$~ & $\ldtwo$ $\pm$ $ \uldtwo$ & 7 \\	

% 	$<\log{R'_{\rm HK}}>$ & $-$4.97 & 8 \\
% % 	P$_{\rm rot}$ [days] & $\prot$  $\pm$  $\prote$ & Huber 2013 \\

% 	P$_{\rm rot}$ [days] & $\prot$  $\pm$  $\prote$ & 7 \\
% 	$\tau_{\rm ev}$ [days] & $\tev$ $\pm$  $\teve$ & 7 \\
% %	Systemic velocity $\gamma~(\ms)$ & $-20926.9^{+0.54}_{-0.64}$ & 5 \\



%  & & \\
% \emph{Transit and radial-velocity parameters} & & & \\
%     Orbital period $P$~[days] & $\perplb$  $\pm$ $ \uperplb $ & 7 \\
%     Time of mid-transit $t_{0}$~[BJD] & $\ttransitb$  $\pm$ \uttransitb & 7\\ 
%     Radius ratio $(R_b/R_\star)$ & $\rprstb$   $\pm$ $ \urprstb$ & 7 \\
%     Orbital inclination $i$~[deg] & $\inclb$   $\pm$ $ \uinclb$ & 7 \\ 
%     Transit impact parameter $b$ & $\impb$   $\pm$ $ \uimpb$ & 7 \\
%     RV semi-amplitude $K$ [m.s$^{-1}$] & $\kamp$   $\pm$ $ ^{\kampeu} _{-\kampel}$ &8 \\
%     RV semi-amplitude 68\% (95\%) upper limit [m.s$^{-1}$] & $<1.8$ ($<2.8$) & 8 \\
%     % RV semi-amplitude 95\% upper limit [m.s$^{-1}$] & $<2.8$ & 8 \\
%     % Eccentricity 68\% upper limit (from transit fit) &$<0.31$ & 7 \\
%     Eccentricity 68\% (95\%) upper limit &$<0.36$ ($<0.79$)& 8 \\  
%     Argument of periastron $\omega_p$ [deg] & -71 $\pm$ 92 & 8 \\
%     RV offset RV$_0$ [km.s$^{-1}$]   & -40.6386 $\pm$ 0.000006 & 8 \\
    
%     % $e_{68\%}<0.31$ and $e_{95\%}<0.71$
                              
%  & & \\
% \emph{Derived parameters for \thisplanet} & & & \\
%     Radius $R_b$~[\rearth] & $\rplb$     $\pm$ $ \urplb$  & 6,7 \\
%     Mass $M_b$~[\mearth] & $\mass$     $\pm$ $ ^{\masseu} _{-\massel}$  & 6,7,8 \\
%     Mass 68\% (95\%) upper limit [\mearth] & $< 6.2$ ($< \mupp$) &        6,7,8 \\
%     % Mass 95\% upper limit [\mearth] & $< \mupp$ &        6,7,8 \\
%     Density $\rho_b$~[g.cm$^{-1}$] & $\rhopl$    $\pm$  $^{\rhopleu} _{-\rhoplel}$  & 6,7,8 \\
%     Density 68\% (95\%) upper limit [g.cm$^{-1}$] & $< 3.2$  ($< 5.1$)  & 6,7,8 \\
%     Scaled semi-major axis $a/R_\star$  & $\arstb$   $\pm$ $\uarstb$ & 7 \\
%     Semi-major axis $a_b$ [AU] & 0.103 $\pm$ 0.001 & 7, 8 \\
%     Incident flux $F$~[\fearth] & $\flux$   $\pm$  $\fluxe$  & 6,7 \\
    


%     & & \\

% \enddata

% 	\tablenotetext{1}{\cite{Hog2000}}
% 	\tablenotetext{2}{\cite{Gaia2016}}
% 	\tablenotetext{3}{from ARES+MOOG analysis, with the surface gravity corrected following \cite{Mortier2014}}
% 	\tablenotetext{4}{Bayesian estimation \citep{Dasilva2006} using the PARSEC isochrones \citep{Bressan2012} and V magnitude and parallax}
% 	\tablenotetext{5}{\cite{Huber2013}}
% 	\tablenotetext{6}{Bayesian estimation using the PARSEC isochrones and asteroseismology}
% 	\tablenotetext{7}{Analysis of the $Kepler$ lightcurve}
% 	\tablenotetext{8}{Analysis of the HARPS-N spectra/RVs}
	
	

% \end{deluxetable*}
% \clearpage
